Learning to Coordinate in a Decentralized Cognitive Radio Network in Presence of Jammers

Efficient utilization of licensed spectrum in the cognitive radio network is challenging due to lack of coordination among the Secondary Users (SUs). Distributed algorithms proposed in the literature aim to maximize the network throughput by ensuring orthogonal channel allocation for the SUs. However, these algorithms work under the assumption that all the SUs faithfully follow the algorithms which may not always hold due to the decentralized nature of the network. In this paper, we study distributed algorithms that are robust against malicious behavior (jamming attack). We consider both the cases of jammers launching coordinated and uncoordinated attacks. In the coordinated attack, the jammers select non-overlapping channels to attack in each time slot and can significantly increase the number of collisions for SUs. We setup the problem in each scenario as a multi-player bandit and develop algorithms. The analysis shows that when the SUs faithfully implement proposed algorithms, the regret is constant with high probability. We validate our claims through exhaustive synthetic experiments and also through a realistic USRP based experiments.

==> Model1s1.tex <==


%		

The regret of the CUJ algorithm is same as the CNJ algorithm.

% Please refer to \cite{TechReport} for proof of the Theorem 3.
 
%\begin{lemma} \label{thm:le5}
%For any $\theta,\epsilon>0$, $\gamma \in (0,\frac{1}{2})$, $\delta \in [0,1]$, $\epsilon_1=\frac{\gamma}{\exp(1).K}$  after 
%$T_C = max (T_{NE},T_{CR}) $ rounds of random exploration, where $T_{NE}=max\left(\frac{8}{\theta}\ln \left(\frac{4K}{\delta_1}\right),\frac{1}{\epsilon^2_1 \theta}\ln \left(\frac{8K}{\delta_1}\right)\right)$, $ T_{CR} = max \left(8K \ln \left(\frac{4K}{\delta_1}\right),\frac{4K}{\epsilon^2}\ln \left ( \frac{8 \cdot K^2}{\delta_1} \right) \right)$ all SUs will have $\epsilon$ correct ranking of channels and all SUs, can estimate N+J with probability atleast $1-\delta_1$. 
%\end{lemma}
%
%Lemma \ref{thm:le5} gives the number of slots required such that all SUs have $\epsilon$ correct ranking of channels and estimate $N+J$ with high probability $1-\delta_1$. In this case, unlike CNJ we have estimate of $N+J$ as we can solve for $N+J$ given in Eq. (\ref{eq:Pc2}). 
%
%\begin{lemma} \label{thm:le6}
%For any $\delta_2 \in [0,1]$, with $T_O = \frac{\log \left(\frac{\delta_2}{K}\right)}{\log \left(1-\left(1-\frac{1}{K} \right) ^ {K-1} \right)}$, all the SUs hopping randomly on $N+J$ chananels will be on orthogonal channels after $T_O$ with probability atleast $1-\delta_2$.
%\end{lemma}
%
%
%Lemma \ref{thm:le6} guarantess that every SU will be on orthogonal channel conditioned that all SUs have estimate of $N+J$ ,after $T_O$ with confidence $1-\delta_2$, where $\delta_2$ is 
%user defined parameter.
%
%\begin{lemma} \label{thm:le7}
%If all SUs are orthogonalised and sequentially hopping on $K$ channels, then for any $\delta_3 \in [0,1]$, $\epsilon_2= \frac
%{\gamma}{Kexp(1)}$, with $T_J = max\left(\frac{8}{\theta }  \cdot \ln \left(\frac{2K}{\delta_3}\right),\frac{1}{\epsilon^2_2 \theta}\ln \left(\frac{4K}{\delta_3}\right)\right)$, all SUs can estimate $\hat{J}=J$ with probability atleast $1-\delta_3$
%\end{lemma}
%
%Lemma \ref{thm:le7} guarantess that given all SUs are orthogonalised as given in lemma \ref{thm:le6}, each SU estimate $J$ with confidence $1-\delta_3$ after $T_J$ rounds.

\begin{thm}\label{thm:t3}
For all  $\Delta > \epsilon$ and $0 \leq\delta\leq 1$, with probability at least $1-\delta$, the expected regret of $N$ SUs using the CUJ algorithm in the presence of $J$ Jammers after $T_L=T_C+T_O+T_J$ time slots of learning is upper bounded by $NT_L + N^2exp(1)$, where the values of $T_C, T_O,$ and $T_J$ are given in  (\ref{eq:TC2}), (\ref{eq:TO2}), and (\ref{eq:TJ2}), respectively with $\epsilon_1=\epsilon_2=\frac{\gamma}{\exp(1).K}$.
\end{thm}
\noindent \textbf{Proof:} \textbf{Channel Ranking Estimation} This part is similar to channel ranking estimation of \ref{thm:le2}. We have,
If \[ T_{CR} = max \left(8K\ln \left(\frac{4K}{\delta_1}\right) ,\frac{4K}{\epsilon^2 }\ln \left ( \frac{8 \cdot K^2}{\delta_1} \right)  \right),\] then for $T_c\geq T_{CR}$ all SUs will have $\epsilon$-correct ranking of channels with probability atleast 
 $1- \frac{\delta_1}{2}.$ 

\noindent \textbf{N+J Estimation:} $W_k$ = event that channel $k$ is selected by a SU \\
$X_k$ = event that none of the other SUs/Jammer selects $k$ \\
$U_k$ = event that channel $k$ is free \\
Let $C_2$ be the number of times we observe that selected channel is free. 
We compute probability of collision given the channel selected is free.
\begin{align*}
Pr(collision) &= \sum\limits_{i=1}^{K}  Pr(W_k/U_k)Pr(X_k/U_k)  \\
p_c	&= \sum\limits_{i=1}^{K} \frac{1}{K} \left(1-\left(1-\frac{1}{K}\right)^{N+J-1} \right)\\
p_c	&= 1-\left(1-\frac{1}{K}\right)^{N+J-1}  \\
\end{align*}

Solving for N+J, 
\[N+J = 1 + \frac{\log \left (1-p_c\right)} {\log \left ( 1-\frac{1}{K} \right )}\] 
Let $\hat{p_c}$  be the estimate of $p_c$. 
\[\overline{N+J} = 1 + \frac{\log \left (1-\hat{p}_c\right)} {\log \left ( 1-\frac{1}{K} \right )}\] 

We want to make $\widehat{N+J}$ as close to $N+J$. Therefore, for $\gamma < \frac{1}{2}$
\[ \left | \widehat{N+J} - N+J \right| < \gamma \] 

\begin{align*}
\left| \frac{\log \left (1-\hat{p}_c\right)} {\log \left ( 1-\frac{1}{K} \right )}-\frac{\log \left (1-p_c\right)} {\log \left ( 1-\frac{1}{K} \right )} \right|  &< \gamma  \\
\left| \frac{\log \left(\frac{1-\hat{p}_c}{1-p_c}\right)}{\log \left ( 1-\frac{1}{K} \right )}\right| &< \gamma  \\
\end{align*}

Let $\alpha$ be the difference between $\hat{p}_c$ and $p_c$. Substituting,
 $\hat{p}_c = p_c +\alpha $.  
\begin{align*}
\left| \frac{\log \left(\frac{1- p_c -\alpha}{1-p_c}\right)}{\log \left ( 1-\frac{1}{K} \right )}\right| &< \gamma
\end{align*}

\begin{align*}
-\gamma\log \left ( 1-\frac{1}{K} \right )&\leq \log \left(\frac{1-p_c - \alpha}{ 1-p_c}  \right) \leq  \gamma\log \left ( 1-\frac{1}{K} \right )
\end{align*}

\begin{align*}
\log \left ( 1-\frac{1}{K} \right )^{-\gamma}&\leq \log \left(\frac{1-p_c - \alpha}{ 1-p_c}  \right) \leq  \log \left ( 1-\frac{1}{K} \right )^\gamma 
\end{align*}

\begin{align*}
 \left ( 1-\frac{1}{K} \right )^{\gamma}&\leq  \left(\frac{1-p_c - \alpha}{ 1-p_c}  \right) \leq   \left ( 1-\frac{1}{K} \right )^{-\gamma}
\end{align*}
\begin{align*}
\left ( 1-\frac{1}{K} \right )^{\gamma} \left(1-p_c \right)&\leq  \left(1-p_c - \alpha  \right) \leq   \left ( 1-\frac{1}{K} \right )^{-\gamma} \left(1-p_c \right) 
\end{align*}
\begin{align*}
\left(1-p_c \right)\left(1-\left ( 1-\frac{1}{K} \right )^{-\gamma} \right) &\leq \alpha \leq \left(1-p_c \right)\left(1-\left ( 1-\frac{1}{K} \right )^{\gamma} \right)
\end{align*}

If we ensure $|\hat{p}_c - p_c| < \epsilon_1$ where
%\begin{equation}\epsilon_1 = min \left \{\left| \left(1-p_c \right)\left(1-\left ( 1-\frac{1}{K} \right )^{-\gamma} \right)\right| \right.,  \left.
%                    \left| \left(1-p_c \right)\left(1-\left ( 1-\frac{1}{K} \right )^{\gamma} \right)\right|\right \}\end{equation}
                    
                    
    \begin{equation*}
\epsilon_1 = min \bigg \{\left| \big (1-p_c \big)\bigg(1-\bigg ( 1-\frac{1}{K} \bigg )^{-\gamma} \bigg)\right|,
\end{equation*}

\begin{equation*}
\left| \big (1-p_c \big)\bigg(1-\bigg ( 1-\frac{1}{K} \bigg )^{\gamma} \bigg)\right| \bigg \}
\end{equation*}                
for some $\gamma<1/2$ then we can have $\widehat{N+J} = N+J$. The number of observations $C_2$ required to compute $\hat{p_c}$
such that $|\hat{p}_c - p_c| < \epsilon_1$ is given by Hoeffding's inequality. 
 \[Pr(|\hat{p}_c - p_c| >\epsilon_1) \leq 2\exp(-2\cdot C_2\cdot\epsilon^2_1) < \frac{\delta_1}{4K} \]
\[\implies C_2 > \frac{1}{2\epsilon^2_1}\ln \left(\frac{8K}{\delta_1}\right) \]

%Find minimum value of epsilon1%
We can further simplify our expression for $\epsilon_1$. Substituing the value of $p_c$, we have 
% \begin{equation}\epsilon_1 = min \left \{\left|\left(1-\frac{1}{K}\right)^{N+J-1} \left(1-\left ( 1-\frac{1}{K} \right )^{-\gamma} \right)\right| , \right. \left.
%                    \left| \left(1-\frac{1}{K}\right)^{N+J-1} \left(1-\left ( 1-\frac{1}{K} \right )^{\gamma} \right)\right|\right \}
%\end{equation}

\begin{equation*}
\epsilon_1 = min \bigg \{\left| \bigg (1-\frac{1}{K}\bigg)^{N+J-1}\bigg(1-\bigg ( 1-\frac{1}{K} \bigg )^{-\gamma} \bigg)\right|,
\end{equation*}

\begin{equation*}
\left| \bigg (1-\frac{1}{K}\bigg)^{N+J-1}\bigg(1-\bigg ( 1-\frac{1}{K} \bigg )^{\gamma} \bigg)\right| \bigg \}
\end{equation*}





Using the results in \cite{MC}, we have 
\[\left|\left(1-\frac{1}{K}\right)^{N+J-1} \left(1-\left ( 1-\frac{1}{K} \right )^{-\gamma} \right)\right| \geq \frac{\gamma}{\exp(1).K}\]
\[\left|\left(1-\frac{1}{K}\right)^{N+J-1} \left(1-\left ( 1-\frac{1}{K} \right )^{\gamma} \right)\right| \geq \frac{\gamma}{\exp(1).K}\]

Therefore, combining above two, we have 

\[\epsilon_1 \geq \frac{\gamma}{\exp(1).K}\]

If we  have $C_2> \frac{1}{2\epsilon^2_1}\ln \left(\frac{8K}{\delta_1}\right) $ observations that the selected channel was free, where $\epsilon_1 =\frac{\gamma}{\exp(1).K}$ then for all SUs with 
probability atleast $1-\frac{\delta_1}{4}$, we have  $\widehat{N+J} = N+J$
\\

Let $A_{I_t}(t)$ be a random variable which indicates if selected channel $k$ is free at round $t$. 
\begin{equation}\label{eq:ct}
				A_{I_t}(t)= \left\{ \begin{array}{cl}
				1& \ if \ selected \ channel \ free \\
				0&  \ otherwise \end{array} \right . 
                \end{equation}

\begin{align*}
E[A_{I_t}(t)] &= \sum\limits_{k=1}^{K}Pr(I_t=k) Pr(A_{I_t}(t)=1/I_t = k) \\
	&= \sum\limits_{k=1}^{K}\frac{1}{K} (1-p_k)\\
	&\geq \theta %\tag{Using $1-p_k \geq \theta \ \forall k \in 1..K$}
\end{align*}
\begin{align*}
Pr &\left(A \ SU \ has < \frac{1}{2}\cdot T_c\cdot E[A_{I_t}(t)] observations\right)  \\ 
 &= Pr\left(\sum\limits_{t=1}^{T_c} A_{I_t}(t) < \frac{1}{2}\cdot T_c\cdot E[A_{I_t}(t)]\right)\\
 &\leq \exp \left(-\frac{1}{8}\cdot T_c\cdot E[A_{I_t}(t)] \right) \tag{Using Chernoff's Bound}
\end{align*}

We want,
\begin{equation*}
Pr \left(SUs \ does \ not \ have \geq \frac{1}{2}T_cE[A_{I_t}(t)] observations\right)
\end{equation*}
\begin{equation*}
< \frac{\delta_1}{4}
\end{equation*}
\begin{align*}
\implies \exp \left(-\frac{1}{8}\cdot T_c\cdot E[A_{I_t}(t)] \right) < \frac{\delta_1}{4K} \\
\implies T_c > 8 \cdot \ln \left(\frac{4K}{\delta_1}\right) \cdot \frac{1}{E[A_{I_t}(t)] } \\ 
\implies T_c > \frac{8}{\theta}\cdot \ln \left(\frac{4K}{\delta_1}\right) 
\end{align*}

We have shown that for $T_c > \frac{8}{\theta}\cdot \ln \left(\frac{4K}{\delta_1}\right)$ , the number of observations of selected channels 
being free for all SUs, $\sum\limits_{t=1}^{T_c} A_{I_t}(t)$ is greater than $ \frac{1}{2}\cdot T_c\cdot E[A_{I_t}(t)]$ with probability atleast
$1-\frac{\delta_1}{4} $


We also want that total number of observations of selected channels being free to be atleast $C_2$.
Therefore, \\ 
\[ \sum\limits_{t=1}^{T_c} A_{I_t}(t) \geq \frac{1}{2}\cdot T_c\cdot E[A_{I_t}(t)] \geq C_2\]
\[\implies \frac{1}{2}\cdot T_c\cdot E[A_{I_t}(t)] > \frac{1}{2\epsilon^2_1}\ln \left(\frac{8K}{\delta_1}\right) \]
\[\implies  T_c > \frac{1}{\epsilon^2_1 E[A_{I_t}(t)]}\ln \left(\frac{8K}{\delta_1}\right) \]
\[\implies  T_c > \frac{1}{\epsilon^2_1 \theta}\ln \left(\frac{8K}{\delta_1}\right) \]
\\
$E$ - event that all SUs have observed atleast $C_2$ times the selected channel was free \\ 
$D$ - event that all SUs have correct estimate of $N$ given $J$ \\


\begin{align*}
Pr(D) &= 1 - Pr(\overline{D})  \\
     &= 1 - Pr(\overline{D}/E)Pr(E) -  Pr(\overline{D}/\overline{E})Pr(\overline{E}) \\
     &\geq 1 - Pr(\overline{D}/E) - Pr(\overline{E}) \\ 
     &\geq 1 - \frac{\delta_1}{4}- \frac{\delta_1}{4}\\
  	&\geq 1 - \frac{\delta_1}{2} 
\end{align*}

If $T_{NE} = max\left(\frac{8}{\theta}\ln \left(\frac{4K}{\delta_1}\right),\frac{1}{\epsilon^2_1 \theta}\ln \left(\frac{8K}{\delta_1}\right)\right)$ then for $T_c \geq T_{NE}$, all SUs would have correct estimate of $N+J$ with probability atleast 
$1-\frac{\delta_1}{2}$ 
\newline
For $A$ and $D$ as defined previously,
\begin{align*}
Pr(AD)&= 1-Pr(\overline{AD}) \\
      &\geq 1 - Pr(\overline{A}) - Pr(\overline{D})\\
      &\geq 1 -  \frac{\delta_1}{2}-\frac{\delta_1}{2}\\
      &\geq 1-\delta_1 
\end{align*}
If $T_c = max (T_{NE},T_{CR})$, then with probability $1-\delta_1$, all SUs would have $\epsilon$-correct channel ranking as well as correct estimate of $N$ given $J$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LEMMA 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

\noindent \textbf{Orthogonalization}
We want to compute $T_O$ such that all SUs are orthogonalised on $N+J$ channels with high probability within $T_O$.
If $p_c$ is the collision probability of a SU at any time slot $t$, and if none of the other SUs are orthogonalized (worst-case) 
then probability that a SUs will find a an orthogonal channel within $T_O$ is given by 
   \begin{equation*} \label{eq:2} \sum\limits_{t=1}^{T_O} p_c^{t-1}\cdot (1-p_c) \end{equation*}.
We want this probability to be atleast $1-\frac{\delta_2}{K}$ to ensure all SUs are orthogonalised within $T_O$.
\begin{align*}
\sum\limits_{t=1}^{T_O} p_c^{t-1}\cdot (1-p_c) &\geq 1-\frac{\delta_2}{K} \\
       1-p_c^{T_O} &\geq 1-\frac{\delta_2}{K}\\
	T_O \log p_c &\leq \log \left(\frac{\delta_2}{K}\right) \\
 T_O &\geq \frac{\log \left(\frac{\delta_2}{K}\right)}{\log p_c} \\
\end{align*}
$p_{ns}$= prob of no collision due to non-settled SUs \\
$p_{s}$= prob of no collision due to settled SUs
\begin{align*}
Pr(no \ collision)
	&= \sum\limits_{k=1}^{N+J}\frac{1}{N+J} (1-p_k) \left(p_{ns}+p_{s}\right) \\ 
   & \left(1-\frac{1}{N+J}\right)^{J} + \sum\limits_{k=1}^{N+J}\frac{p_k}{N+J}\\
	 p_{nc}&\geq \sum\limits_{k=1}^{N+J}\frac{1}{N+J} (1-p_k) \left(p_{ns}+p_{s}\right)\\
	 &\left(1-\frac{1}{N+J}\right)^{J}\\
    &\geq \sum\limits_{k=1}^{N+J}\frac{1}{N+J} (1-p_k) p_{ns}\left(1-\frac{1}{N+J}\right)^{J}\\
    &\geq \sum\limits_{k=1}^{N+J}\frac{1}{N+J} (1-p_k) \left(1-\frac{1}{N+J} \right)^{N+J-1} \\
    &\geq \theta\left(1-\frac{1}{N+J} \right)^{N+J-1} \\ 
  &\geq \theta\left(1-\frac{1}{K} \right)^{K-1}\\
  p_c  &\leq 1-\theta\left(1-\frac{1}{K} \right)^{K-1}\\ 
\implies T_O &\geq \frac{\log \left(\frac{\delta_2}{K}\right)}{\log \left(1-\theta\left(1-\frac{1}{K} \right) ^ {K-1} \right)} \\
\end{align*}
Now, SUs will be randomly hopping on $N+J$ channels and jammers will be attacking top $N+J$ channels. 

To compute the settling time, we upper bound the collision probability as follows:
	
F - an event that all SUs are orthogonalised given all SUs have correct estimate of $N+J$.
We just showed that $Pr(F) \geq  1-\delta_2.$

\noindent \textbf{Jammer Estimation}
The SUs are orthogonalised and locked themselves on top $N+J$ channels.
We want to compute $T_J$, slots required to estimate $J$ correctly with high probability.
Given $C_3$ number of observations that the channel was free, we will estimate $J$ by computing collision probablities
only during the channel is free.

\begin{align*}
Pr(collision)=p_c &= 1-\left(1-\frac{1}{N+J}\right)^J \\
\end{align*} 	
Solving for $J$,
\[J = \frac{\log \left (1-p_c\right)} {\log \left ( 1-\frac{1}{N+J} \right )}\] 
Let $\hat{p_c}$  be the estimate of $p_c$. 
\[\hat{J} =  \frac{\log \left (1-\hat{p}_c\right)} {\log \left ( 1-\frac{1}{N+J} \right )}\] 

We want to make $\hat{J}$ as close to $J$. Therefore, for $\gamma < \frac{1}{2}$
\[ \left | \hat{J} - J \right| < \gamma \] 

\begin{align*}
\left| \frac{\log \left (1-\hat{p}_c\right)} {\log \left ( 1-\frac{1}{N+J} \right )}-\frac{\log \left (1-p_c\right)} {\log \left ( 1-\frac{1}{N+J} \right )} \right|  &< \gamma  \\
\left| \frac{\log \left(\frac{1-\hat{p}_c}{1-p_c}\right)}{\log \left ( 1-\frac{1}{N+J} \right )}\right| &< \gamma  \\
\end{align*}

Let $\alpha$ be the difference between $\hat{p}_c$ and $p_c$. Substituting,
 $\hat{p}_c = p_c +\alpha $.  
%\[\left| \frac{\log \left(\frac{1- p_c -\alpha}{1-p_c}\right)}{\log \left ( 1-\frac{1}{N+J} \right )}\right| < \gamma  \\
% -\gamma\log \left ( 1-\frac{1}{N+J} \right )\leq \log \left(\frac{1-p_c - \alpha}{ 1-p_c}  \right) \leq  \gamma\log \left ( 1-\frac{1}{N+J} \right )\]
\[\log \left ( 1-\frac{1}{N+J} \right )^{-\gamma}\leq \log \left(\frac{1-p_c - \alpha}{ 1-p_c}  \right) \leq  \log \left ( 1-\frac{1}{N+J} \right )^\gamma \]
\[\left ( 1-\frac{1}{N+J} \right )^{\gamma}\leq  \left(\frac{1-p_c - \alpha}{ 1-p_c}  \right) \leq   \left ( 1-\frac{1}{N+J} \right )^{-\gamma}\]
\[\left ( 1-\frac{1}{N+J} \right )^{\gamma} \left(1-p_c \right)\leq  \left(1-p_c - \alpha  \right) \leq   \left ( 1-\frac{1}{N+J} \right )^{-\gamma} \left(1-p_c \right)\]

\begin{equation*}\left(1-p_c \right)\left(1-\left ( 1-\frac{1}{N+J} \right )^{-\gamma} \right) \leq \alpha \leq \end{equation*}
\begin{equation} \leq \left(1-p_c \right)\left(1-\left ( 1-\frac{1}{N+J} \right )^{\gamma} \right)\end{equation}
If we ensure $|\hat{p}_c - p_c| < \epsilon_2$ where
%\begin{equation}\epsilon_2= min \left \{\left| \left(1-p_c \right)\left(1-\left ( 1-\frac{1}{N+J} \right )^{-\gamma} \right)\right| , 
%            \right.   \left.      \left| \left(1-p_c \right)\left(1-\left ( 1-\frac{1}{N+J} \right )^{\gamma} \right)\right|\right \}
%\end{equation}

\begin{equation*}
\epsilon_1 = min \bigg \{\left| \big(1-p_c\big) \bigg(1-\bigg ( 1-\frac{1}{N+J} \bigg )^{-\gamma} \bigg)\right|,
\end{equation*}

\begin{equation*}
\left| \big(1-p_c\big)\bigg(1-\bigg ( 1-\frac{1}{N+J} \bigg )^{\gamma} \bigg)\right| \bigg \}
\end{equation*}

for some $\gamma<1/2$ then we can have $\hat{J} = J$. The number of observations $C_3$ required to compute $\hat{p_c}$
such that $|\hat{p}_c - p_c| \leq \epsilon_2$ is given by Hoeffding's inequality. 
 \[Pr(|\hat{p}_c - p_c| >\epsilon_2) \leq 2\exp(-2\cdot C_3\cdot\epsilon^2_2) < \frac{\delta_3}{2K} \]
\[\implies C_3 > \frac{1}{2\epsilon^2_2}\ln \left(\frac{4K}{\delta_3}\right) \]

%Find minimum value of epsilon1%
We can further simplify our expression for $\epsilon_1$. Substituing the value of $p_c$, we have 
% \begin{equation}\epsilon_2 = min \left \{\left|\left(1-\frac{1}{N+J}\right)^{J} \left(1-\left ( 1-\frac{1}{N+J} \right )^{-\gamma} \right)\right| , 
%         \right.    \left.       \left| \left(1-\frac{1}{N+J}\right)^{J} \left(1-\left ( 1-\frac{1}{N+J} \right )^{\gamma} \right)\right|\right \}
%\end{equation}

\begin{equation*}
\epsilon_1 = min \bigg \{\left| \bigg (1-\frac{1}{N+J}\bigg)^{J} \bigg(1-\bigg ( 1-\frac{1}{N+J} \bigg )^{-\gamma} \bigg)\right|,
\end{equation*}

\begin{equation*}
\left| \bigg (1-\frac{1}{N+J}\bigg)^{J} \bigg(1-\bigg ( 1-\frac{1}{N+J} \bigg )^{\gamma} \bigg)\right| \bigg \}
\end{equation*}


Using the results in \cite{MC}, we have 
\[\left|\left(1-\frac{1}{N+J}\right)^{J} \left(1-\left ( 1-\frac{1}{N+J} \right )^{-\gamma} \right)\right| \geq \frac{\gamma}{\exp(1).K}\]
\[\left|\left(1-\frac{1}{N+J}\right)^{J} \left(1-\left ( 1-\frac{1}{N+J} \right )^{\gamma} \right)\right| \geq \frac{\gamma}{\exp(1).K}\]

Therefore, combining above two, we have 
\[
\epsilon_2 \geq \frac{\gamma}{\exp(1).K}\]

If we  have $C_3> \frac{1}{2\epsilon^2_2}\ln \left(\frac{4K}{\delta_3}\right)  $ observations that the selected channel was free, where $\epsilon_2 =\frac{\gamma}{\exp(1).K}$ then for all SUs with 
probability atleast $1-\frac{\delta_3}{2}$, we have  $\hat{J} = J$

To ensure we have $C_3$ observations of selected channels being free for all users, using similar approach as in proof of lemma \ref{thm:le1} used for $N+J$ estimation, we can say ,
   
\begin{align*}
Pr \left(all \ SUs \ has < \frac{1}{2}\cdot T_J\cdot E[A_{I_t}(t)] observations\right)< \frac{\delta_3}{2} \\
\implies \exp \left(-\frac{1}{8}\cdot T_J\cdot E[A_{I_t}(t)] \right) < \frac{\delta_3}{2K} \\
\implies T_J > 8 \cdot \ln \left(\frac{2K}{\delta_3}\right) \cdot \frac{1}{E[A_{I_t}(t)] }  
\end{align*}

where $T_J$ is the number of slots for Jammer Estimation. In this case, $E[A_k(t)] = 1-p_k$.
We also want that total number of observations of selected channels being free to be atleast $C_3$.
Therefore, \\ 
\[ \sum\limits_{t=1}^{T_J} A_{I_t}(t) \geq \frac{1}{2}\cdot T_J\cdot E[A_{I_t}(t)] \geq C_3\]
\[\implies \frac{1}{2}\cdot T_J\cdot E[A_{I_t}(t)] > \frac{1}{2\epsilon^2_2}\ln \left(\frac{4K}{\delta_3}\right)\]
\[\implies  T_J > \frac{1}{\epsilon^2_2 E[A_{I_t}(t)]}\ln \left(\frac{4K}{\delta_3}\right) \]

\noindent $G$ - event that all SUs have observed atleast $C_3$ times the selected channel was free \\ 
$G_n$ - event that $n^{th}$ SU has observed atleast $C_3$ times the selected channel was free \\
$H$ - event that all SUs have correct estimate of $J$ given all SUs are orthogonalised when selected channel was free \\
$H_n$ - event that $n^{th}$ SU has correct estimate of $N$ given all SUs are orthogonalised when selected channel was free \\

\begin{align*}
Pr(H) &= 1 - Pr(\overline{H})  \\
     &= 1 - Pr(\overline{H}/G)Pr(G) -  Pr(\overline{H}/\overline{E})Pr(\overline{E}) \\
     &\geq 1 - Pr(\overline{H}/G) - Pr(\overline{G}) \\ 
     &\geq 1 - \sum\limits_{n=1}^{N} Pr(\overline{H_n}/G_n) - \sum\limits_{n=1}^{N} Pr(\overline{G_n})  \tag{Union Bound}\\  	
     &\geq 1 - 	\sum\limits_{n=1}^{N} \frac{\delta_3}{2K}-\sum\limits_{n=1}^{N} \frac{\delta_3}{2K}\\
     &\geq 1 - \frac{\delta_3}{K}N \\
 	&\geq 1 - \frac{\delta_1}{K}K \\
  	&\geq 1 - \delta_3 \\
\end{align*}

\noindent Let Y be an event that all SUs have correct estimate of $N$ and $J$ as well as they are orthogonalised and have correct channel ranking.
\begin{align*}
Pr(Y) &\geq Pr(Y/ADFH)\cdot Pr(ADFH)  \\
   &\geq Pr(Y/ADFH)\cdot Pr(H/ADF)\cdot Pr(ADF) \\ 
   &\geq Pr(Y/ADFH)\cdot Pr(H/ADF)\cdot Pr(F/AD) \cdot Pr(AD) \\ 
\end{align*}

 We have, 
\begin{equation*}
   \geq Pr(Y/ADFH)\cdot Pr(H/ADF)\cdot Pr(F/AD) \cdot Pr(AD) 
\end{equation*}
   \begin{equation*}
Pr(Y)  \geq (1-\delta_3)(1-\delta_2)(1-\delta_1) 
\end{equation*}

Setting $ \delta_1 = \delta_2=\delta_3=\frac{\delta}{3}$ 

\begin{equation*}
Pr(Y)  \geq \left(1-\frac{\delta}{3}\right)^3 
\end{equation*}
\begin{equation*}
Pr(Y)  \geq 1-3\frac{\delta}{3}
\end{equation*}
\begin{equation*}
Pr(Y)  \geq 1-\delta
\end{equation*}

\noindent Now, to bound regret consider following:
if $(m<=J)$: \\
\begin{align*}
Pr(no \ collision)
	&= \sum\limits_{k=1}^{N+m}\frac{(1-p_k)}{N+m}  \left(p_{ns}+p_{s}\right)\left(1-\frac{1}{N+J}\right)^{J} \\
	&+\sum\limits_{k=1}^{N+m}\frac{p_k}{N+m}\\
p_{nc}&\geq \sum\limits_{k=1}^{N+m}\frac{(1-p_k)}{N+m}  \left(p_{ns}+p_{s}\right)\left(1-\frac{1}{N+J}\right)^{J}\\
    &\geq \sum\limits_{k=1}^{N+m}\frac{(1-p_k)}{N+m}  p_{ns}\left(1-\frac{1}{N+J}\right)^{J}\\
    &\geq \sum\limits_{k=1}^{N+m}\frac{(1-p_k)}{N+m}  \left(1-\frac{1}{N+m} \right)^{N-1}\left(1-\frac{1}{N+J} \right)^{J} \\
    &\geq \theta\left(1-\frac{1}{N+J} \right)^{N+J-1} \\ 
  &\geq \theta\left(1-\frac{1}{K} \right)^{K-1}\\
\end{align*}

if $(m>J)$: \\
\begin{align*}
Pr(no \ collision)
	&= \sum\limits_{k=1}^{N+J}\frac{(1-p_k)}{N+m}  \left(p_{ns}+p_{s}\right)\left(1-\frac{1}{N+J}\right)^{J} \\ 
    &+\sum\limits_{k=N+J+1}^{N+m}\frac{(1-p_k)}{N+m}  \left(p_{ns}+p_{s}\right)\\
    &+ \sum\limits_{k=1}^{N+m}\frac{p_k}{N+m}\\
p_{nc}&\geq \sum\limits_{k=1}^{N+m}\frac{(1-p_k)}{N+m}  \left(p_{ns}+p_{s}\right)\left(1-\frac{1}{N+J}\right)^{J}\\
    &\geq \sum\limits_{k=1}^{N+m}\frac{(1-p_k)}{N+m}  p_{ns}\left(1-\frac{1}{N+J}\right)^{J}\\
    &\geq \sum\limits_{k=1}^{N+m}\frac{(1-p_k)}{N+m}  \left(1-\frac{1}{N+m} \right)^{N-1}\\
    &\left(1-\frac{1}{N+J} \right)^{J} \\
    &\geq \theta\left(1-\frac{1}{N+m} \right)^{N+J-1} \\ 
  &\geq \theta\left(1-\frac{1}{K} \right)^{K-1}\\
    &\geq \frac{\theta}{exp(1)} 
\end{align*}
Combining above two cases, we can say 
\[p_{nc} \geq \frac{\theta}{exp(1)}\]
\[\implies T_f\leq \frac{exp(1)}{\theta}\]
Regret will again be bounded as $NT_f$, i.e., 
$\frac{N^2exp(1)}{\theta}$. Hence proving theorem \ref{thm:t3}







==> Model2s1.tex <==
%%Non_distinguishable collision






%The following theorem states the expected regret of the CNJ against the jammers who employs Algorithm \ref{Algo2}. Again the expectation is over the randomness of the algorithm.
%\begin{thm}\label{thm:t2}
%For all 
%	$\Delta > \epsilon, \gamma \in (0,0.5)$ and $0 < \delta\leq 1$, with probability at least $1-\delta$, the expected regret of SUs using CNJ in the presence of $J$ jammers after $T_L=T_C+T_O+T_J$ slots of learning is upper bounded by $NT_L + N^2exp(1)$, where
%	\begin{eqnarray}
%	\nonumber
%	T_{C}&=&\mbox{round} \bigg (\max\bigg(\frac{8}{\theta}\ln \left(\frac{12K}{\delta}\right),\frac{1}{\epsilon^2_1 \theta}\ln \left(\frac{24K}{\delta}\right) ,\\
%	\label{eq:TC2}
%	&& \hspace{1cm}8K \ln \left(\frac{12K^2}{\delta}\right),
%	\frac{4K}{\epsilon^2}\ln \left ( \frac{24K^2}{\delta} \right) \bigg)\bigg)\\
%		\label{eq:TO2}
%	T_O &=&\mbox{round}\bigg(\frac{\log \left(\frac{\delta}{3K}\right)}{\log \left(1-\frac{\theta}{K}\left(1-\frac{1}{K} \right) ^	{K-1} \right)} \bigg )\\
%		\label{eq:TJ2}
%	T_J &=& \hspace{-.2cm}\mbox{round} \bigg (max\left(\frac{8}{\theta }  \ln \left(\frac{6K}{\delta}\right),\frac{1}{\epsilon^2_2 \theta}\ln \left(\frac{12K}{\delta}\right)\right)\bigg)
%	\end{eqnarray}
%with $\epsilon_1=\frac{\gamma}{2\exp(1).K}$ and $\epsilon_2= \frac
%{\gamma}{K}$.
%\end{thm}
%\noindent
%The terms $NT_C, NT_O, NT_J$ correspond to the total regret incurred by all the players in the first three subroutines, i.e., CR2, OR and JE respectively. The last term corresponds to the OR subroutine that runs till the end of time horizon. The theorem is proved using the following lemmas which give the number of time slots required to estimate the parameters with high confidence. 
\begin{lemma} \label{thm:le2}
For any $\delta>0$, all SUs will have $\epsilon$-correct ranking of channels and   $\hat{N}=N$ given $J$ with probability at least $1-\delta/3$ if CR2 subroutine is run for $T_C$ number of time slots.
\end{lemma}
\noindent \textbf{Proof:} \textbf{Channel Ranking Estimation}
If for any player $n$ it is true that $\forall k \in 1 \cdots K$ $\left | \hat{p}_k-p_k \right| \leq\frac{\epsilon}{2} $ then the 
player has an  $\epsilon-$ correct ranking.

We will upper bound the probability that no player has $\epsilon-$ correct ranking given the player have $C$ observations of each 
channel. 
We define the following events : \\

\noindent$J_n$ - event that a player $n$ has observed each channel $j\geq0$ times.\\
$A$ - event that all players have an $\epsilon$-correct ranking. \\
$A_n$ - event that a player $n$ has $\epsilon$- correct ranking. \\
$B$ - event that all players have atleast $C$ observations of each channel. \\
$B_n$ - event that a player $n$ has atleast $C$ observations of each channel. \\ 

Note*: $\overline{X}$ denotes complement of any event $X$\\


We want to compute,
\[Pr(\overline{A}_n|B_n) < \frac{\delta_1}{4K} \]

Also, we know , 
\begin{align*}
Pr(\overline{A}_n|B_n) &\leq Pr\left ( \exists k \in 1 \cdots K \ \ s.t | \hat{p}_k-p_k | >\frac{\epsilon}{2} | \ B_n\right) \\
 \tag{By Union Bound}      &\leq \sum_{k=1}^{K} Pr\left ( | \hat{p}_k-p_k | >\frac{\epsilon}{2} | \ B_n\right) \\ 
       			&= \sum_{k=1}^{K} \sum_{j=C}^{\infty} Pr\left (| \hat{p}_k-p_k | >\frac{\epsilon}{2} | \ 
J_n  \right) Pr \left( J_n | \ B_n \right) \\ 
 \tag {By Hoeffding's Inequality} &\leq \sum_{k=1}^{K} \sum_{j=C}^{\infty} 2 \cdot \exp \left(\frac{-j \cdot \epsilon^2}{2} \right) Pr \left( J_n | \ B_n \right) \\ 
	&\leq \sum_{k=1}^{K} 2 \cdot \exp \left(\frac{-C \cdot \epsilon^2}{2} \right) \sum_{j=C}^{\infty} Pr \left( J_n | \ B_n \right) \\ 
	 &\leq \sum_{k=1}^{K} 2 \cdot \exp \left(\frac{-C \cdot \epsilon^2}{2} \right)  \\
	 &\leq K \cdot 2 \cdot \exp \left(\frac{-C \cdot \epsilon^2}{2} \right)
\end{align*}

We can apply Hoeffding's Inequality since each observation of the channel is independent of the number of times we observe that
channel.This is true since each SU is randomly selecting channels in CR phase, which is independent of the
previous rounds.In order for this to be $< \frac{\delta_1}{4K}$, 
	 \[ K \cdot 2 \cdot \exp \left(\frac{-C \cdot \epsilon^2}{2} \right) < \frac{\delta_1}{4K} \newline
		\implies  C >   \ln \left ( \frac{8 \cdot K^2}{\delta_1} \cdot  \right) \frac{2}{\epsilon^2}
\]

%If each player $i$ has $ C =  \ln \left ( \frac{2 \cdot K \cdot (K)}{\delta_1} \cdot  \right) \frac{2}{\epsilon^2}$ observations of each 
%channel then with probability atleast $1-\frac{\delta_1}{K}$, player $i$ will have an $\epsilon-$ correct ranking of channels.

Now, to show that if all players have at least $ C > \ln \left ( \frac{8 \cdot K^2}{\delta_1} \cdot  \right) \frac{2}{\epsilon^2}$ observations of each channel, then all players have an $\epsilon-$ correct ranking of channels with probability atleast $1-\frac{\delta_1}{4}$. 

\begin{align*} 
     Pr(A|B) &\geq 1-Pr\left( \vee_n Pr(\overline{A}_n | B_n) \right) \\
            &\geq 1-\sum_{n=1}^{N} Pr(\overline{A}_n | B_n)    \tag{By Union Bound}\\
	    &\geq 1-\frac{\delta_1}{4K} \cdot (N) \\
            &\geq 1-\frac{\delta_1}{4K} \cdot K\\
	    &= 1-\frac{\delta_1}{4}
\end{align*}


We want to show that there exists a $T_c$ large enough such that all SUs have greater than $C$ observations of each channel.  
Let $B_{n,k}(t)$ be a random variable which indicates that channel $k$ is selected by a player $n$. 
\begin{equation*}\label{eq:ct}
				B_{n,k}(t)= \left\{ \begin{array}{cl}
				1 &\ w.p \ \frac{1}{K} \\
				0 &\ w.p \ \frac{1}{K} \end{array} \right . 
                \end{equation*}
\[E\left[B_{n,k}(t)\right] = \frac{1}{K} \]

\begin{align*}
Pr &\left(A \ SU \ has < \frac{1}{2}\cdot T_c\cdot E[B_{n,k}(t) observations\right)  \\ 
 &= Pr\left(\sum\limits_{t=1}^{T_c} B_{n,k}(t) < \frac{1}{2}\cdot T_c\cdot E[B_{n,k}(t)]\right)\\
 &\leq \exp \left(-\frac{1}{8}\cdot T_c\cdot B_{n,k}(t)] \right) \tag{Using Chernoff's Bound}
\end{align*}

We want,
\begin{align*}
Pr \left(\exists n,k \ s.t.\sum\limits_{t=1}^{T_c} B_{n,k}(t) < \frac{1}{2}\cdot T_c\cdot E[B_{n,k}(t)]\right)  <\frac{\delta_1}{4} \\
\implies N\exp \left(-\frac{1}{8}\cdot T_c\cdot E[B_{n,k}(t)] \right) < \frac{\delta_1}{4K} \\
\implies T_c > 8 \cdot \ln \left(\frac{4K^2}{\delta_1}\right) \cdot \frac{1}{E[B_{n,k}(t)] } \\
\implies T_c > 8K\ln \left(\frac{4K^2}{\delta_1}\right)
\end{align*}

We have shown that for $T_c >8K\ln \left(\frac{4K^2}{\delta_1}\right)$ , the number of observations of selected channels for all SUs, $\sum\limits_{t=1}^{T_c} B_{n,k}(t)$ is greater than $ \frac{1}{2}\cdot T_c\cdot E[B_{n,k}(t)]$ with probability atleast
$1-\frac{\delta_1}{4} $

We also want that total number of observations of each channel be atleast $C$.
Therefore, \\ 
\[ \sum\limits_{t=1}^{T_c} B_{n,k}(t) \geq \frac{1}{2}\cdot T_c\cdot E[B_{n,k}(t)] \geq C\]
\[\implies \frac{1}{2}\cdot T_c\cdot E[B_{n,k}(t)] \geq \ln \left ( \frac{8 \cdot K^2}{\delta_1}\right) \frac{2}{\epsilon^2} \]
\[\implies  T_c \geq \frac{4}{\epsilon^2 E[B_{n,k}(t)]}\ln \left ( \frac{8 \cdot K^2}{\delta_1} \right)    \]
\[\implies  T_c \geq \frac{4K}{\epsilon^2 }\ln \left ( \frac{8 \cdot K^2}{\delta_1} \right)    \]

\begin{align*}
Pr(A) &= 1 - Pr(\overline{A}) \\
      &= 1 - Pr(\overline{A}/B)Pr(B)-Pr(\overline{A}/\overline{B})Pr(\overline{B}) \\
      &\geq 1 - Pr(\overline{A}/B) - Pr(\overline{B})\\
      &\geq 1- \frac{\delta_1}{4} - \frac{\delta_1}{4} \\
      &\geq 1- \frac{\delta_1}{2}
\end{align*}
If $ T_{CR} = max \left(8K\ln \left(\frac{4K^2}{\delta_1}\right),\frac{4K}{\epsilon^2}\ln \left ( \frac{8 \cdot K^2}{\delta_1} \right) \right)$, then for $T_c\geq T_{CR}$ all SUs will have $\epsilon$-correct ranking of channels with probability atleast 
 $1- \frac{\delta_1}{2}.$ 

%%%%%%%%%%%%%%%%% N Estimation %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55

\noindent \textbf{N Estimation:} $W_k$ = event that channel $k$ is selected by a SU \\
$X_k$ = event that none of the other SUs/Jammer selects $k$ \\
$U_k$ = event that channel $k$ is free \\
Let $C_2$ be the number of times we observe that selected channel is free. 
We compute probability of collision given the channel selected is free and the number of Jammers $J$.
\begin{align*}
Pr(collision) &= \sum\limits_{k=1}^{K}  Pr(W_k/U_k)Pr(X_k/U_k)  \\
p_c	&= \sum\limits_{k=1}^{K} \frac{1}{K} \left(1-\left(1-\frac{J}{K}\right)\left(1-\frac{1}{K}\right)^{N-1}  \right)\\
p_c	&= 1-\left(1-\frac{J}{K}\right)\left(1-\frac{1}{K}\right)^{N-1}   \\
\end{align*}

Solving for N, 
\[N = 1 + \frac{\log \left (1-p_c\right)-\log \left ( 1-\frac{J}{K} \right )} {\log \left ( 1-\frac{1}{K} \right )}\] 
Let $\hat{p_c}$  be the estimate of $p_c$. 
\[\hat{N} = 1 + \frac{\log \left (1-\hat{p}_c\right)-\log \left ( 1-\frac{J}{K} \right )} {\log \left ( 1-\frac{1}{K} \right )}\] 

We want to make $\hat{N}$ as close to $N$. Therefore, for $\gamma < \frac{1}{2}$
\[ \left | \hat{N} - N \right| < \gamma \] 

\begin{align*}
\left| \frac{\log \left (1-\hat{p}_c\right)} {\log \left ( 1-\frac{1}{K} \right )}-\frac{\log \left (1-p_c\right)} {\log \left ( 1-\frac{1}{K} \right )} \right|  &< \gamma  \\
\left| \frac{\log \left(\frac{1-\hat{p}_c}{1-p_c}\right)}{\log \left ( 1-\frac{1}{K} \right )}\right| &< \gamma  \\
\end{align*}

Let $\alpha$ be the difference between $\hat{p}_c$ and $p_c$. Substituting,
 $\hat{p}_c = p_c +\alpha $.  

\begin{align*}
\left| \frac{\log \left(\frac{1- p_c -\alpha}{1-p_c}\right)}{\log \left ( 1-\frac{1}{K} \right )}\right| &< \gamma  
\end{align*}
\begin{align*}
-\gamma\log \left ( 1-\frac{1}{K} \right ) \leq \log \left(\frac{1-p_c - \alpha}{ 1-p_c}  \right) \leq  \gamma\log \left ( 1-\frac{1}{K} \right )
\end{align*}
\begin{align*}
\log \left ( 1-\frac{1}{K} \right )^{-\gamma}&\leq \log \left(\frac{1-p_c - \alpha}{ 1-p_c}  \right) \leq  \log \left ( 1-\frac{1}{K} \right )^\gamma 
\end{align*}
 \begin{align*}
  \left ( 1-\frac{1}{K} \right )^{\gamma}&\leq  \left(\frac{1-p_c - \alpha}{ 1-p_c}  \right) \leq   \left ( 1-\frac{1}{K} \right )^{-\gamma}
 \end{align*}
  \begin{align*}
  \left ( 1-\frac{1}{K} \right )^{\gamma} \left(1-p_c \right)&\leq  \left(1-p_c - \alpha  \right) \leq   \left ( 1-\frac{1}{K} \right )^{-\gamma} \left(1-p_c \right)
   \end{align*}
   \begin{align*}
\left(1-p_c \right)\left(1-\left ( 1-\frac{1}{K} \right )^{-\gamma} \right) &\leq \alpha \leq \left(1-p_c \right)\left(1-\left ( 1-\frac{1}{K} \right )^{\gamma} \right)
\end{align*}

If we ensure $|\hat{p}_c - p_c| < \epsilon_1$ where
%\begin{equation*}
%\epsilon_1 = min \left \{\left| \left(1-p_c \right)\left(1-\left ( 1-\frac{1}{K} \right )^{-\gamma} \right)\right| ,  \right.\left. 
%							\left| \left(1-p_c \right)\left(1-\left ( 1-\frac{1}{K} \right )^{\gamma} \right)\right|\right \}
%\end{equation*}

\begin{equation*}
\epsilon_1 = min \bigg \{\left| \big (1-p_c \big)\bigg(1-\bigg ( 1-\frac{1}{K} \bigg )^{-\gamma} \bigg)\right|,
\end{equation*}

\begin{equation*}
\left| \big (1-p_c \big)\bigg(1-\bigg ( 1-\frac{1}{K} \bigg )^{\gamma} \bigg)\right| \bigg \}
\end{equation*}

%\begin{equation}
%\right.\left. \left| \left(1-p_c \right)\left(1-\left ( 1-\frac{1}{K} \right )^{\gamma} \right)\right|\right \}
%\end{equation}
for some $\gamma<1/2$ then we can have $\hat{N} = N$. The number of observations $C_2$ required to compute $\hat{p_c}$
such that $|\hat{p}_c - p_c| \leq \epsilon_1$  for all SUs is given by Hoeffding's inequality. 
 \[Pr(|\hat{p}_c - p_c| >\epsilon_1) \leq 2\exp(-2\cdot C_2\cdot\epsilon^2_1) < \frac{\delta_1}{4K} \]
\[\implies C_2 > \frac{1}{2\epsilon^2_1}\ln \left(\frac{8K}{\delta_1}\right) \]

%Find minimum value of epsilon1%
We can further simplify our expression for $\epsilon_1$. Substituing the value of $p_c$, we have 
% \begin{equation}\epsilon_1 = min \left \{\left|\left(1-\frac{1}{K}\right)^{N-1} \left(1-\frac{J}{K} \right) \left(1-\left ( 1-\frac{1}{K} \right )^{-\gamma} \right)\right| ,\right.  \left.
%                    \left| \left(1-\frac{1}{K}\right)^{N-1} \left(1-\frac{J}{K} \right) \left(1-\left ( 1-\frac{1}{K} \right )^{\gamma} \right)\right|\right \}
% \end{equation}
 
 \begin{equation*}
\epsilon_1 = min \bigg \{\left| \bigg (1-\frac{1}{K}\bigg)^{N-1}\bigg(1-\frac{J}{K}\bigg) \bigg(1-\bigg ( 1-\frac{1}{K} \bigg )^{-\gamma} \bigg)\right|,
\end{equation*}

\begin{equation*}
\left| \bigg (1-\frac{1}{K}\bigg)^{N-1}\bigg(1-\frac{J}{K}\bigg) \bigg(1-\bigg ( 1-\frac{1}{K} \bigg )^{\gamma} \bigg)\right| \bigg \}
\end{equation*}
 
 
 
 
Using the results in \cite{MC} and  $\left(1-\frac{J}{K} \right)\geq \frac{1}{2}$  as $K>N>J$ ,we have 
\[\left|\left(1-\frac{1}{K}\right)^{N-1} \left(1-\frac{J}{K} \right)\left(1-\left ( 1-\frac{1}{K} \right )^{-\gamma} \right)\right| \geq \frac{\gamma}{2\exp(1)K}\]
\[\left|\left(1-\frac{1}{K}\right)^{N-1}\left(1-\frac{J}{K} \right) \left(1-\left ( 1-\frac{1}{K} \right )^{\gamma} \right)\right| \geq \frac{\gamma}{2\exp(1)K}\]
Therefore, combining above two, we have 

\[\epsilon_1 \geq \frac{\gamma}{2\exp(1).K}\]

If all SUs have $C_2>\frac{1}{2\epsilon^2_1}\ln \left(\frac{8K}{\delta_1}\right)$ observations that the selected channel was free, where $\epsilon_1 =\frac{\gamma}{2\exp(1).K}$ then with 
probability atleast $1-\frac{\delta_1}{4}$, we have  $\hat{N} = N$ for all SUs
\\

We want to show that there exists a $T_c$ large enough such that all SUs have greater than $C_2$ observations of selected channel were 
free. 
Let $A_{I_t}(t)$ be a random variable which indicates if selected channel $k$ is free at round $t$. 
\begin{equation}\label{eq:ct}
				A_{I_t}(t)= \left\{ \begin{array}{cl}
				1& \ if \ selected \ channel \ free \\
				0&  \ otherwise \end{array} \right . 
                 \end{equation}

\begin{align*}
E[A_{I_t}(t)] &= \sum\limits_{k=1}^{K}Pr(I_t=k) Pr(A_{I_t}(t)=1/I_t = k) \\
	&= \sum\limits_{k=1}^{K}\frac{1}{K} (1-p_k)\\
	&\geq \theta %\tag{Using $1-p_k \geq \theta \ \forall k \in 1..K$}
\end{align*}
\begin{align*}
Pr &\left(A \ SU \ has < \frac{1}{2}\cdot T_c\cdot E[A_{I_t}(t)] observations\right)  \\ 
 &= Pr\left(\sum\limits_{t=1}^{T_c} A_{I_t}(t) < \frac{1}{2}\cdot T_c\cdot E[A_{I_t}(t)]\right)\\
 &\leq \exp \left(-\frac{1}{8}\cdot T_c\cdot E[A_{I_t}(t)] \right) \tag{Using Chernoff's Bound}
\end{align*}

We want,
\begin{align*}
Pr \left(SUs \ does \ not \ have > \frac{1}{2} T_cE[A_{I_t}(t)] observations\right)< \frac{\delta_1}{4} \\
\implies \exp \left(-\frac{1}{8}\cdot T_c\cdot E[A_{I_t}(t)] \right) < \frac{\delta_1}{4K} \\
\implies T_c > 8 \cdot \ln \left(\frac{4K}{\delta_1}\right) \cdot \frac{1}{E[A_{I_t}(t)] } \\ 
\implies T_c > \frac{8}{\theta}\cdot \ln \left(\frac{4K}{\delta_1}\right) 
\end{align*}

We have shown that for $T_c > \frac{8}{\theta}\cdot \ln \left(\frac{4K}{\delta_1}\right)$ , the number of observations of selected channels 
being free for all SUs, $\sum\limits_{t=1}^{T_c} A_{I_t}(t)$ is greater than $ \frac{1}{2}\cdot T_c\cdot E[A_{I_t}(t)]$ with probability atleast
$1-\frac{\delta_1}{4} $


We also want that total number of observations of selected channels being free to be atleast $C_2$.
Therefore, \\ 
\[ \sum\limits_{t=1}^{T_c} A_{I_t}(t) \geq \frac{1}{2}\cdot T_c\cdot E[A_{I_t}(t)] \geq C_2\]
\[\implies \frac{1}{2}\cdot T_c\cdot E[A_{I_t}(t)] \geq \frac{1}{2\epsilon^2_1}\ln \left(\frac{8K}{\delta_1}\right) \]
\[\implies  T_c \geq \frac{1}{\epsilon^2_1 E[A_{I_t}(t)]}\ln \left(\frac{8K}{\delta_1}\right) \]
\[\implies  T_c \geq \frac{1}{\epsilon^2_1 \theta}\ln \left(\frac{8K}{\delta_1}\right) \]
\\
$E$ - event that all SUs have observed atleast $C_2$ times the selected channel was free \\ 
$D$ - event that all SUs have correct estimate of $N$ given $J$ \\


\begin{align*}
Pr(D) &= 1 - Pr(\overline{D})  \\
     &= 1 - Pr(\overline{D}/E)Pr(E) -  Pr(\overline{D}/\overline{E})Pr(\overline{E}) \\
     &\geq 1 - Pr(\overline{D}/E) - Pr(\overline{E}) \\ 
     &\geq 1 - \frac{\delta_1}{4}- \frac{\delta_1}{4}\\
  	&\geq 1 - \frac{\delta_1}{2} 
\end{align*}

If $T_{NE} = max\left(\frac{8}{\theta}\ln \left(\frac{4K}{\delta_1}\right),\frac{1}{\epsilon^2_1 \theta}\ln \left(\frac{8K}{\delta_1}\right)\right)$ then for $T_c \geq T_{NE}$, all SUs would have correct estimate of $N$ given $J$ with probability atleast 
$1-\frac{\delta_1}{2}$ 
\newline
For $A$ and $D$ as defined previously,
\begin{align*}
Pr(AD)&= 1-Pr(\overline{AD}) \\
      &\geq 1 - Pr(\overline{A}) - Pr(\overline{D})\\
      &\geq 1 -  \frac{\delta_1}{2}-\frac{\delta_1}{2}\\
      &\geq 1-\delta_1 
\end{align*}
If $T_c = max (T_{NE},T_{CR})$, then with probability $1-\delta_1$, all SUs would have $\epsilon$-correct channel ranking as well as correct estimate of $N$ given $J$.
%Note that $N$ estimation is conditioned on the event that $J$ is known. As the probability of collision depends both on $N$ and $J$ as given in (\ref{eq:PC}), to estimate $N$, $J$ should be known a priori. This is why in Algorithm \ref{Algo3} we store collision data during CR2 phase and estimate $N$ only after estimating $J$ in JE phase. 
\begin{lemma} \label{thm:le3}
For any $\delta>0$, all SUs will find non-overlapping channels with probability at least $1-\delta/3$ if OR subroutine is run for $T_O$ number of time slots.
\end{lemma}
%\noindent \textbf{Proof:} We want to compute $T_O$ such that all SUs are orthogonalized on $K$ channels with high probability within $T_O$.
%If $p_c$ is the collision probability of a SU at any time slot $t$, and if none of the other SUs are orthogonalized (worst-case) 
%then probability that a SUs will find a an orthogonal channel within $T_O$ is given by 
%   \begin{equation*} \label{eq:2} \sum\limits_{t=1}^{T_O} p_c^{t-1}\cdot (1-p_c) \end{equation*}.
%We want this probability to be atleast $1-\frac{\delta_2}{K}$ for every SU to ensure all SUs are orthogonalized within $T_O$ with probability $1-\delta$.
%\begin{align*}
%\sum\limits_{t=1}^{T_O} p_c^{t-1}\cdot (1-p_c) &\geq 1-\frac{\delta_2}{K} \\
%       1-p_c^{T_O} &\geq 1-\frac{\delta_2}{K}\\
%	T_O \log p_c &\leq \log \left(\frac{\delta_2}{K}\right) \\
% T_O &\geq \frac{\log \left(\frac{\delta_2}{K}\right)}{\log p_c} \\
%\end{align*}
%
%Now, SUs will be randomly hopping on $K$ channels and jammers will be attacking top $N$ channels. \\
%$p_{ns}$= probability of no collision due to non-settled SUs \\
%$p_{s}$= probability of no collision due to settled SUs
%\begin{align*}
%Pr(no \ collision)
%	&= \sum\limits_{k=1}^{N}\frac{1}{K} (1-p_k) \left(p_{ns}+p_{s}\right)\left(1-\frac{J}{N}\right) \\ 
%  &+ \sum\limits_{k=N+1}^{K}\frac{1}{K} (1-p_k) \left(p_{ns}+p_{s}\right) + \sum\limits_{k=1}^{K}\frac{p_k}{K}\\
% p_{nc} &\geq \sum\limits_{k=1}^{K}\frac{1}{K} (1-p_k) \left(p_{ns}+p_{s}\right)\left(1-\frac{J}{N}\right)\\
%    &\geq \sum\limits_{k=1}^{K}\frac{1}{K} (1-p_k) p_{ns}\left(1-\frac{J}{N}\right)\\
%    &\geq \sum\limits_{k=1}^{K}\frac{1}{K} (1-p_k) \left(1-\frac{1}{K} \right)^{N-1}\left(1-\frac{J}{N}\right) \\
%    &\geq \left(1-\frac{1}{K} \right)^{N-1}\left(\frac{N-J}{N}\right) \theta\\  \tag{Using $\sum\limits_{K=1}^{K} \frac{1}{K}(1-p_k) \geq \theta \  \& \ N>J$}
%  &\geq \left(1-\frac{1}{K} \right)^{K-1}\left(\frac{1}{N}\right) \theta\\ 
%    &\geq \left(1-\frac{1}{K} \right)^{K-1}\left(\frac{1}{K}\right) \theta\\ 
%\end{align*}
%
%Note that when we lower bound $p_{ns}$, we consider the worst case that all SUs are not settled.
%\begin{align*}
%p_c &= 1-p_{nc} \\
%p_c &\leq 1-\left(1-\frac{1}{K} \right)^{K-1}\left(\frac{1}{K}\right) \theta \\
%\implies T_O &\geq \frac{\log \left(\frac{\delta_2}{K}\right)}{\log \left(1-\frac{\theta}{K}\left(1-\frac{1}{K} \right) ^ {K-1} \right)} \\
%\end{align*} 	
%
%F - an event that all SUs are orthogonalized. We just showed that a SU gets orthogonalized with probability $1-\frac{\delta_2}{K}$. Therefore, all SUs would get orthogonalized with probability atleast $1-\delta_2$, i.e., $Pr(F) \geq  1-\delta_2.$
\begin{lemma} \label{thm:le4}
For any $\delta>0$, all SUs will estimate $\hat{J}=J$ with probability at least $1-\delta/3$ if JE subroutine is run for $T_J$ number of time slots.
\end{lemma}
\noindent \textbf{Proof:} Given that SUs are orthogonalized on $K$ channels we want to compute number of slots required to estimate $J$ correctly with high probability for all SUs. 
We will compute collision probability only when the channel is free.
Let $C_3$ be the number of times we observe that selected channel is free after orthogonalization.
Given $C_3$, we want to ensure correct estimation of $J$ with high probability.
We also assume that jammer is hitting top $N$ channels.
\begin{align*} {\label{eq:Pc4}}
Pr(collision) = p_c &= \sum\limits_{i=1}^{N} \frac{1}{K} \left(1-1-\frac{J}{N}\right) \\
 p_c &= \sum\limits_{i=1}^{N} \frac{1}{K} \frac{J}{N} \\
p_c = \frac{J}{K} \\
\implies J = Kp_c
\end{align*}

Let $\hat{p}_c$ be the estimate of $p_c$. Then estimate of $J$ is given by, \\
\[\hat{J}=K\hat{p}_c \]

We want to ensure $\hat{J}$ is close to $J$. Therefore, for some $\gamma < 1/2$ 
\begin{align*} 
\left| \hat{J}- J \right| &\leq \gamma \\
\left| \hat{p}_c - p_c \right| &\leq \frac{\gamma}{K} \\
\end{align*}

The number of observations $C_3$ required to compute $\hat{p_c}$
such that $|\hat{p}_c - p_c| \leq \epsilon_2$, where $\epsilon_2= \frac{\gamma}{K}$ for all SUs is given by Hoeffding's inequality. 
 \[Pr(|\hat{p}_c - p_c| >\epsilon_2) \leq 2\exp(-2\cdot C_3\cdot\epsilon^2_2) < \frac{\delta_3}{2K} \]
\[\implies C_3 > \frac{1}{2\epsilon^2_2}\ln \left(\frac{4K}{\delta_3}\right) \]

To ensure we have $C_3$ observations of selected channels being free for all users, we define $A_{I_t}(t)$ and $E[A_{I_t}(t)] \geq \theta$ 
as defined in proof of lemma \ref{thm:le1} used for $N$ and $J$ estimation. 
   \begin{equation*}
   Pr \left(all \ SUs \ does \ not \ have \geq \frac{1}{2} T_JE[A_{I_t}(t)] observations\right)
   \end{equation*}
   \begin{equation*}
 < \frac{\delta_3}{2}
   \end{equation*}
\begin{align*}
\implies \exp \left(-\frac{1}{8}\cdot T_J\cdot E[A_{I_t}(t)] \right) < \frac{\delta_3}{2K} \\
\implies T_J > 8 \cdot \ln \left(\frac{2K}{\delta_3}\right) \cdot \frac{1}{E[A_{I_t}(t)] }  \\
\implies T_J > \frac{8}{\theta }  \cdot \ln \left(\frac{2K}{\delta_3}\right)
\end{align*}

where $T_J$ is the number of slots for Jammer Estimation.
We also want that total number of observations of selected channels being free to be atleast $C_3$.
Therefore, \\ 
\[ \sum\limits_{t=1}^{T_J} A_{I_t}(t) \geq \frac{1}{2}\cdot T_J\cdot E[A_{I_t}(t)] \geq C_3\]
\[\implies \frac{1}{2}\cdot T_J\cdot E[A_{I_t}(t)] > \frac{1}{2\epsilon^2_2}\ln \left(\frac{4K}{\delta_3}\right)\]
\[\implies  T_J > \frac{1}{\epsilon^2_2 E[A_{I_t}(t)]}\ln \left(\frac{4K}{\delta_3}\right) \]
\[\implies  T_J > \frac{1}{\epsilon^2_2 \theta}\ln \left(\frac{4K}{\delta_3}\right) \]
\[T_J = max\left(\frac{8}{\theta }  \cdot \ln \left(\frac{2K}{\delta_3}\right),\frac{1}{\epsilon^2_2 \theta}\ln \left(\frac{4K}{\delta_3}\right)\right) \]
$G$ - event that all SUs have observed atleast $C_3$ times the selected channel was free \\ 
$H$ - event that all SUs have correct estimate of $J$\\


\begin{align*}
Pr(H) &= 1 - Pr(\overline{H})  \\
     &= 1 - Pr(\overline{H}/G)Pr(G) -  Pr(\overline{H}/\overline{E})Pr(\overline{E}) \\
     &\geq 1 - Pr(\overline{H}/G) - Pr(\overline{G}) \\ 
     &\geq 1 - \frac{\delta_3}{2}- \frac{\delta_3}{2}\\
  	&\geq 1 - \delta_3 \\
\end{align*}
%\texttt{The proofs of these lemmas are again based on careful applications of Hoeffding's inequality and Chernoff bound and appropriately bounding the collision probabilities. For more details see \cite{TechReport}.} 

The following theorem states the expected regret of the CNJ against the jammers who employs the jamming strategy as in CDJ. Again the expectation is over the randomness of the algorithm.
\begin{thm}\label{thm:t2}
For all 
	$\Delta > \epsilon, \gamma \in (0,0.5)$ and $0 < \delta\leq 1$, with probability at least $1-\delta$, the expected regret of SUs using CNJ in the presence of $J$ jammers after $T_L=T_C+T_O+T_J$ slots of learning is upper bounded by $NT_L + N^2exp(1)$, where
	
	\begin{equation*}
	T_{C}=\mbox{round} \bigg (\max\bigg(\frac{8}{\theta}\ln \left(\frac{12K}{\delta}\right),\frac{1}{\epsilon^2_1 \theta}\ln \left(\frac{24K}{\delta}\right)
	\end{equation*}
	\begin{equation}
	, \ln \left(\frac{12K^2}{\delta}\right), \frac{4K}{\epsilon^2}\ln \left ( \frac{24K^2}{\delta} \right) \bigg)\bigg)\\
	\label{eq:TC2}
	\end{equation}
	\begin{eqnarray}	 
		\label{eq:TO2}
	T_O &=&\mbox{round}\bigg(\frac{\log \left(\frac{\delta}{3K}\right)}{\log \left(1-\frac{\theta}{K}\left(1-\frac{1}{K} \right) ^	{K-1} \right)} \bigg )\\
		\label{eq:TJ2}
	T_J &=& \hspace{-.2cm}\mbox{round} \bigg (max\left(\frac{8}{\theta }  \ln \left(\frac{6K}{\delta}\right),\frac{1}{\epsilon^2_2 \theta}\ln \left(\frac{12K}{\delta}\right)\right)\bigg)
	\end{eqnarray}
with $\epsilon_1=\frac{\gamma}{2\exp(1).K}$ and $\epsilon_2= \frac
{\gamma}{K}$.
\end{thm}
\noindent
The terms $NT_C, NT_O, NT_J$ correspond to the total regret incurred by all the players in the first three subroutines, i.e., CR2, OR and JE respectively. The last term corresponds to the OR subroutine that runs till the end of time horizon.
% The theorem is proved using the following lemmas which give the number of time slots required to estimate the parameters with high confidence. 

\noindent \textbf{Proof:} Let Y be an event that all SUs have correct estimate of $N$ and $J$ as well as they are orthogonalized and have correct channel ranking after $T_L$ learning rounds.
Let $M$ be an event that all SUs have correct estimate of $N$.
A,D,F,H are as defined in proof of lemmas \ref{thm:le2}, \ref{thm:le3}, \ref{thm:le4}
\begin{align*}
Pr(Y) &\geq Pr(Y/AMFH)\cdot Pr(AMFH)  \\
   &\geq Pr(Y/AMFH)\cdot Pr(AM/FH)\cdot Pr(FH) \\ 
   &\geq Pr(Y/AMFH)\cdot Pr(AD)\cdot PR(H/F)\cdot Pr(F) \\  \tag{event $M$ given $H$ is $D$}
\end{align*}

Using Lemmas \ref{thm:le2},\ref{thm:le3},\ref{thm:le4} , we have, 
\begin{equation*}
Pr(Y)  \geq Pr(Y/AMFH)Pr(AD)PR(H/F)Pr(F)
\end{equation*}
\begin{equation*}
Pr(Y)  \geq (1-\delta_1)(1-\delta_3)(1-\delta_2) 
\end{equation*}
Setting $ \delta_1 = \delta_2=\delta_3=\frac{\delta}{3}$ 
\begin{equation*}
Pr(Y)  \geq \left(1-\frac{\delta}{3}\right)^3 
\end{equation*}
\begin{equation*}
Pr(Y)  \geq 1-3\frac{\delta}{3}
\end{equation*}
\begin{equation*}
Pr(Y)  \geq 1-\delta
\end{equation*}

Setting $T_L = T_C + T_O+T_J$, with probability atleast $1-\delta$, all SUs have correct estimate of $N$ and $J$ as well as they are orthogonalized and have correct channel ranking.

Substituting value of $\delta_1,\delta_2,\delta_3$, we have,
\begin{equation*}
T_C= max \bigg(\frac{8}{\theta}\ln \bigg(\frac{12K}{\delta}\bigg), \frac{1}{\epsilon^2_1 \theta}\ln \bigg(\frac{24K}{\delta}\bigg), 8K\ln \left(\frac{12K^2}{\delta}\right),
\end{equation*}

\begin{equation*}
\frac{4K}{\epsilon^2}\ln \left ( \frac{24 \cdot K^2}{\delta} \right) \bigg)
\end{equation*}
\[ T_O=\frac{\log \left(\frac{\delta}{3K}\right)}{\log \left(1-\frac{\theta}{k}\left(1-\frac{1}{K} \right) ^ {K-1} \right)} \]
\[T_J=max\left(\frac{8}{\theta }  \cdot \ln \left(\frac{6K}{\delta}\right),\frac{1}{\epsilon^2_2 \theta}\ln \left(\frac{12K}{\delta}\right) \right)\]

Regret bounds proof is similar to proof of 
Theorem $1$. 

==> Model3s1.tex <==
%%%%Distinguishable collisions



In this section, we bound the regret of CDJ. We begin with the following definition given in \cite{MC,MEGA}.
\begin{defn}
An $\epsilon$-correct ranking of $K$ channels is a sorted list of empirical mean values of channel occupancy probabilities such that for all $i,j$, $\hat{p}_i$ is listed before $\hat{p}_j$ if $p_j - p_i >  \epsilon$.
\end{defn}
\noindent

\begin{lemma} \label{thm:le1}
By the end of CR1 phase, all SUs have $\epsilon$-correct ranking of the channels, number of SUs (N) and Jammer $J$ with probability at least $1-\delta$.
\end{lemma}
%\noindent \textbf{Proof}: The proof steps are similar to \cite{MC}[Lemma 1].
%If for any player $n$ it is true that $\forall k \in 1 \cdots K$ $\left | \hat{p}_k-p_k \right| \leq\frac{\epsilon}{2} $ then the 
%player has an  $\epsilon-$ correct ranking. We will upper bound the probability that no player has $\epsilon-$ correct ranking given the player have $C$ observations of each 
%channel. 
%We define the following events : \\
%
%\noindent$J_n$ - event that player $n$ observed each channel $j\geq0$ times.\\
%$A$ - event that all players have an $\epsilon$-correct ranking. \\
%$A_n$ - event that a player $n$ has $\epsilon$- correct ranking. \\
%$B$ - event that all players have atleast $C$ observations of each channel. \\
%$B_n$ - event that a player $n$ has atleast $C$ observations of each channel. Let $\overline{X}$ denote complement of any event $X$\\
%
%We first upper bound $Pr(\overline{A}_n|B_n)$. We have, 
%\begin{align*}
%Pr(\overline{A}_n|B_n) &\leq Pr\left ( \exists k \in 1 \cdots K \ \ s.t | \hat{p}_k-p_k | >\frac{\epsilon}{2} | \ B_n\right) \\
% \tag{By Union Bound}      &\leq \sum_{k=1}^{K} Pr\left ( | \hat{p}_k-p_k | >\frac{\epsilon}{2} | \ B_n\right) \\ 
%       			&= \sum_{k=1}^{K} \sum_{j=C}^{\infty} Pr\left (| \hat{p}_k-p_k | >\frac{\epsilon}{2} | \ 
%J_n  \right) Pr \left( J_n | \ B_n \right) \\ 
% \tag {By Hoeffding's Inequality} &\leq \sum_{k=1}^{K} \sum_{j=C}^{\infty} 2  \exp \left(\frac{-j  \epsilon^2}{2} \right) Pr \left( J_n | \ B_n \right) \\ 
%	&\leq \sum_{k=1}^{K} 2  \exp \left(\frac{-C  \epsilon^2}{2} \right) \sum_{j=C}^{\infty} Pr \left( J_n | \ B_n \right) \\ 
%	 &\leq \sum_{k=1}^{K} 2 \exp \left(\frac{-C \epsilon^2}{2} \right) \leq K  2  \exp \left(\frac{-C \epsilon^2}{2} \right)
%\end{align*}
%We can apply Hoeffding's inequality since each observation of the channel is independent of the number of times we observe that
%channel. This is true since each SU and jammer is randomly selecting channels independent of the
%previous rounds in each round. In order for this to be $< \frac{\delta}{4K}$, 
%	 \[ K 2  \exp \left(\frac{-C  \epsilon^2}{2} \right) < \frac{\delta}{4K} \newline
%		\implies  C >   \ln \left ( \frac{8  K^2}{\delta}   \right) \frac{2}{\epsilon^2}
%\]
%
%%If each player $i$ has $ C =  \ln \left ( \frac{2 \cdot K \cdot (K)}{\delta} \cdot  \right) \frac{2}{\epsilon^2}$ observations of each 
%%channel then with probability atleast $1-\frac{\delta}{K}$, player $i$ will have an $\epsilon-$ correct ranking of channels.
%Now to show that if all players have at least $ C > \ln \left ( \frac{8  K^2}{\delta}   \right) \frac{2}{\epsilon^2}$ observations of each channel, then all players have an $\epsilon-$ correct ranking of channels with probability atleast $1-\frac{\delta}{4}$. 
%
%\begin{align*} 
%     Pr(A|B) &\geq 1-Pr\left( \vee_n Pr(\overline{A}_n | B_n) \right) \\
%            &\geq 1-\sum_{n=1}^{N} Pr(\overline{A}_n | B_n)    \tag{By Union Bound}\\
%	    &\geq 1-\frac{\delta}{4K}  (N) \geq 1-\frac{\delta}{4K}  K= 1-\frac{\delta}{4}
%\end{align*}
%We want to show that there exists a $T_c$ large enough such that all SUs have greater than $C$ observations of each channel.  
%Let $B_{n,k}(t)$ be a random variable which indicates that channel $k$ is selected by SU $n$. 
%\begin{equation*}\label{eq:ct}
%				B_{n,k}(t)= \left\{ \begin{array}{cl}
%				1 &\ w.p \ \frac{1}{K} \\
%				0 &\ w.p \ \frac{1}{K}. \end{array} \right .
%                \end{equation*}
% We have   
%\begin{align*}
%Pr &\left(\ SU \ n \ has < \frac{1}{2} T_c E[B_{n,k}(t)] \ observations\right)  \\ 
% &= Pr\left(\sum\limits_{t=1}^{T_c} B_{n,k}(t) < \frac{1}{2}T_c E[B_{n,k}(t)]\right)\\
% &\leq \exp \left(-\frac{1}{8} T_c E[B_{n,k}(t)] \right) \tag{ Chernoff's Bound}
%\end{align*}
%We can apply Chernoff bound here since for any n,k, $B_{n,k}$ is i.i.d across t, since all SUs employ random sampling in CR phase.
%We want,
%\begin{align*}
%&Pr \left(\exists n,k \ s.t.\sum\limits_{t=1}^{T_c} B_{n,k}(t) < \frac{1}{2} T_c E[B_{n,k}(t)]\right) <\frac{\delta}{4} \\
%&\implies N\exp \left(-\frac{1}{8} T_c E[B_{n,k}(t)] \right) < \frac{\delta}{4K} \\
%&\implies T_c > 8  \ln \left(\frac{4KN}{\delta}\right)  \frac{1}{E[B_{n,k}(t)] } \\
%&\implies T_c > 8  \ln \left(\frac{4K^2}{\delta}\right)  \frac{1}{E[B_{n,k}(t)] } \\
%&\implies T_c > 8K\ln \left(4K^2/\delta\right)
%\end{align*}
%The last inequality follows using $E\left[B_{n,k}(t)\right] = 1/K$. We have shown that for $T_c >8K\ln \left(4K^2/\delta\right)$ , the number of observations of selected channels for all SUs, $\sum\limits_{t=1}^{T_c} B_{n,k}(t)$ is greater than $ \frac{1}{2} T_c E[B_{n,k}(t)]$ with probability atleast
%$1-\frac{\delta}{4} $. We also want that total number of observations of each channel be atleast $C$. Therefore,
%\begin{align*}
%&\sum\limits_{t=1}^{T_c} B_{n,k}(t) \geq \frac{1}{2} T_c E[B_{n,k}(t)] \geq C\\
%&\implies \frac{1}{2}T_c E[B_{n,k}(t)] \geq \ln \left ( \frac{8  K^2}{\delta}\right) \frac{2}{\epsilon^2}\\
%&\implies  T_c \geq \frac{4}{\epsilon^2 E[B_{n,k}(t)]}\ln \left ( \frac{8  K^2}{\delta} \right)    \\
%&\implies  T_c \geq \frac{4K}{\epsilon^2 }\ln \left ( \frac{8  K^2}{\delta} \right)   
%\end{align*}
%Combining all, the probability that all the players will have $\epsilon$-correct ranking is given by
%\begin{align*}
%Pr(A) &= 1 - Pr(\overline{A}) \\
%      &= 1 - Pr(\overline{A}/B)Pr(B)-Pr(\overline{A}/\overline{B})Pr(\overline{B}) \\
%      &\geq 1 - Pr(\overline{A}/B) - Pr(\overline{B})\geq 1- \frac{\delta}{4} - \frac{\delta}{4} \geq 1- \frac{\delta}{2}.
%\end{align*}
%Thus, if $ T_{CR} = \max \left(8K\ln \left(\frac{4K^2}{\delta}\right),\frac{4K}{\epsilon^2}\ln \left ( \frac{8  K^2}{\delta} \right) \right)$, then for $T_c\geq T_{CR}$ all SUs will have $\epsilon$-correct ranking of channels with probability atleast 
% $1- \frac{\delta}{2}.$ 
%
% 
%%%%%%%%%%%%%%%%%% no of user estimation%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%\noindent \textbf{Estimation of $N$}: Now, we compute number of slots required to estimate $N$ and $J$ with high probability.
%We first compute slots required to estimate $N$ given $J$. We define the following events : \\
%
%\noindent$W_k$ - event that channel $k$ is selected by a SU \\
%$X_k$ - event that none of the other SUs/Jammer selects $k$ \\
%$U_k$ - event that channel $k$ is free. \\
%
%\noindent
%Let $C_2$ be the number of times a selected channel is found free. 
%Probability of collision, denoted $p_c$, for any SU conditioned on the events that the channel selected is free and the number of Jammers is $J$ is given by
%\begin{align*}
%Pr(collision) &= \sum\limits_{k=1}^{K}  Pr(W_k/U_k)Pr(X_k/U_k)  \\
%p_c	&= \sum\limits_{k=1}^{K} \frac{1}{K} \left(1-\left(1-\frac{J}{K}\right)\left(1-\frac{1}{K}\right)^{N-1}  \right)\\
%p_c	&= 1-\left(1-\frac{J}{K}\right)\left(1-\frac{1}{K}\right)^{N-1}   \\
%\end{align*}
%Solving for N, we get
%\[N = 1 + \frac{\log \left (1-p_c\right)-\log \left ( 1-\frac{J}{K} \right )} {\log \left ( 1-\frac{1}{K} \right )}\] 
%Let $\hat{p_c}$  be the estimate of $p_c$. 
%\[\hat{N} = 1 + \frac{\log \left (1-\hat{p}_c\right)-\log \left ( 1-\frac{J}{K} \right )} {\log \left ( 1-\frac{1}{K} \right )}\] 
%We want $\hat{N}$ to be a good estimate of $N$. Therefore, for some $\gamma < \frac{1}{2}$, we set $ \left | \hat{N} - N \right| < \gamma$
%  
%\[\left| \frac{\log \left (1-\hat{p}_c\right)} {\log \left ( 1-\frac{1}{K} \right )}-\frac{\log \left (1-p_c\right)} {\log \left ( 1-\frac{1}{K} \right )} \right|  < \gamma  \iff \left| \frac{\log \left(\frac{1-\hat{p}_c}{1-p_c}\right)}{\log \left ( 1-\frac{1}{K} \right )}\right| < \gamma   \]
%Let $\alpha$ be the difference between $\hat{p}_c$ and $p_c$. Substituting $\hat{p}_c = p_c +\alpha $.  
%
%\[-\gamma\log \left ( 1-\frac{1}{K} \right )\leq \log \left(\frac{1-p_c - \alpha}{ 1-p_c}  \right) \leq  \gamma\log \left ( 1-\frac{1}{K} \right )  \]
%\[ \log \left ( 1-\frac{1}{K} \right )^{-\gamma}\leq \log \left(\frac{1-p_c - \alpha}{ 1-p_c}  \right) \leq  \log \left ( 1-\frac{1}{K} \right )^\gamma \]
%\[ \left ( 1-\frac{1}{K} \right )^{\gamma}\leq  \left(\frac{1-p_c - \alpha}{ 1-p_c}  \right) \leq   \left ( 1-\frac{1}{K} \right )^{-\gamma} \]
%\[ \left ( 1-\frac{1}{K} \right )^{\gamma} \left(1-p_c \right)\leq  \left(1-p_c - \alpha  \right) \leq   \left ( 1-\frac{1}{K} \right )^{-\gamma} \left(1-p_c \right)  \]
%\[ \left(1-p_c \right)\left(1-\left ( 1-\frac{1}{K} \right )^{-\gamma} \right) \leq \alpha \leq \left(1-p_c \right)\left(1-\left ( 1-\frac{1}{K} \right )^{\gamma} \right). \]
%If we ensure $|\hat{p}_c - p_c| < \epsilon_1$ where
%\begin{equation}\epsilon_1 = \min \left \{\left| \left(1-p_c \right)\left(1-\left ( 1-\frac{1}{K} \right )^{-\gamma} \right)\right| \right.,
% \left. \left| \left(1-p_c \right)\left(1-\left ( 1-\frac{1}{K} \right )^{\gamma} \right)\right|\right \}\end{equation}
%for some $\gamma<1/2$ then we can have $\hat{N} = N$. The number of observations $C_2$ required to compute $\hat{p_c}$
%such that $|\hat{p}_c - p_c| \leq \epsilon_1$  for all SUs is given by Hoeffding's inequality. 
% \[Pr(|\hat{p}_c - p_c| >\epsilon_1) \leq 2\exp(-2 C_2\epsilon^2_1) < \frac{\delta}{6K} \]
%\[\implies C_2 > \frac{1}{2\epsilon^2_1}\ln \left(\frac{12K}{\delta}\right) \]
%Following steps in the proof of \cite{MC}, we can further simplify the expression for $\epsilon_1$. Substituting the value of $p_c$, we have 
% \begin{equation}\epsilon_1 = \min \left \{\left|\left(1-\frac{1}{K}\right)^{N-1} \left(1-\frac{J}{K} \right) \left(1-\left ( 1-\frac{1}{K} \right )^{-\gamma} \right)\right| \right., \left.
%                    \left| \left(1-\frac{1}{K}\right)^{N-1} \left(1-\frac{J}{K} \right) \left(1-\left ( 1-\frac{1}{K} \right )^{\gamma} \right)\right|\right \}\end{equation}
%Using $\left(1-\frac{J}{K} \right)\geq \frac{1}{2}$  as $K>N>J$, we have 
%\[\left|\left(1-\frac{1}{K}\right)^{N-1} \left(1-\frac{J}{K} \right)\left(1-\left ( 1-\frac{1}{K} \right )^{-\gamma} \right)\right| \geq \frac{\gamma}{2\exp(1)K}\]
%\[\left|\left(1-\frac{1}{K}\right)^{N-1}\left(1-\frac{J}{K} \right) \left(1-\left ( 1-\frac{1}{K} \right )^{\gamma} \right)\right| \geq \frac{\gamma}{2\exp(1)K}\]
%Combining above two, we have 
%\[\epsilon_1 \geq \frac{\gamma}{2\exp(1)K}\]
%If all SUs have $C_2>\frac{1}{2\epsilon^2_1}\ln \left(\frac{12K}{\delta}\right)$ observations of channel when they are free, where $\epsilon_1 =\frac{\gamma/K}{2\exp(1)}$, then with 
%probability at least $1-\frac{\delta}{6}$, we have  $\hat{N} = N$ for all SUs given $J$.\\
%
%\textbf{Estimation of $J$:} Next we compute number of slots required to estimate $J$ correctly by all SUs with high probability. 
%We compute collision probability with jammers when the channel is free.
%Let $C_3$ be the number of times we observe that selected channel is free.
%Given $C_3$, we want to ensure correct estimation of $J$ with high probability.
%\begin{align*} {\label{eq:Pc4}}
%Pr(jammer \; from\; collision) = p_{cj }&= \sum\limits_{i=1}^{K} \frac{1}{K} \left(\frac{J}{K}\right) \\
%\implies J = Kp_{cj}
%\end{align*}
%Let $\hat{p}_{cj}$ be the estimate of $p_{cj}$. Then the estimate of $J$ is given by $\hat{J}=K\hat{p}_{cj}$.
%We want to ensure $\hat{J}$ is close to $J$. Therefore, for some $\gamma < 1/2$ 
%\begin{align*} 
%\left| \hat{J}- J \right| \leq \gamma 
%\iff \left| \hat{p}_{cj} - p_{cj} \right| \leq \frac{\gamma}{K} \\
%\end{align*}
%The number of observations $C_3$ required to compute $\hat{p_{cj}}$
%such that $|\hat{p}_{cj} - p_{cj}| \leq \epsilon_2$, where $\epsilon_2= \frac{\gamma}{K}$ for all SUs is given by applying the Hoeffding's inequality. 
% \[Pr(|\hat{p}_{cj }- p_{cj}| >\epsilon_2) \leq 2\exp(-2 C_3\epsilon^2_2) < \frac{\delta}{12K} \]
%\[\implies C_3 > \frac{1}{2\epsilon^2_2}\ln \left(\frac{24K}{\delta}\right) \]
%We next show that there exists a $T_c$ large enough such that all SUs have greater than $C_2$ observations of selected channel were 
%free. 
%Let $A_{I_t}(t)$ be a random variable which indicates if selected channel $k$ is free at round $t$. 
%\begin{equation}\label{eq:ct}
%				A_{I_t}(t)= \left\{ \begin{array}{cl}
%				1& \mbox{ if  $I_t$  is free}\\
%				0&   \mbox{otherwise} \end{array} \right . 
%                \end{equation}
%We have
%\begin{align*}
%Pr &\left(a \ SU \ has < \frac{1}{2}\cdot T_c\cdot E[A_{I_t}(t)] observations\right)  \\ 
% &= Pr\left(\sum\limits_{t=1}^{T_c} A_{I_t}(t) < \frac{1}{2}\cdot T_c\cdot E[A_{I_t}(t)]\right)\\
% &\leq \exp \left(-\frac{1}{8}\cdot T_c\cdot E[A_{I_t}(t)] \right) \tag{ Chernoff's Bound}
%\end{align*}
%We want,
%\begin{align*}
%&Pr \left(all \ SUs \ does \ not \ have > \frac{1}{2} T_cE[A_{I_t}(t)] observations\right)< \frac{\delta}{18} \\
%&\implies \exp \left(-\frac{1}{8} T_c E[A_{I_t}(t)] \right) < \frac{\delta}{18K} \\
%&\implies T_c > 8  \ln \left(\frac{18K}{\delta}\right)  \frac{1}{E[A_{I_t}(t)] } \\ 
%&\implies T_c >\frac{8}{\theta}  \ln \left(\frac{18K}{\delta}\right),  
%\end{align*}
%In the last if-and-only statement we used
%\begin{align*}
%E[A_{I_t}(t)] &= \sum\limits_{k=1}^{K}Pr(I_t=k) Pr(A_{I_t}(t)=1/I_t = k) \\
%&= \sum\limits_{k=1}^{K}\frac{1}{K} (1-p_k)\geq \theta. 
%\end{align*}
%We have shown that for $T_c > \frac{8}{\theta} \cdot \ln \left(\frac{18K}{\delta}\right)  $ , the number of observations of 
%selected channels being free for all SUs, $\sum\limits_{t=1}^{T_c} A_{I_t}(t)$ is greater than $ \frac{1}{2}\cdot T_c\cdot E[A_{I_t}(t)]$ 
%with probability atleast $1-\frac{\delta}{18} $
%
%We also want that total number of observations of selected channels being free to be atleast $C_2$ and $C_3$ .
%Therefore, \\ 
%\[ \sum\limits_{t=1}^{T_c} A_{I_t}(t) \geq \frac{1}{2}\cdot T_c\cdot E[A_{I_t}(t)] \geq C_2\]
%\[\implies \frac{1}{2}\cdot T_c\cdot E[A_{I_t}(t)] \geq \frac{1}{2\epsilon^2_1}\ln \left(\frac{12K}{\delta}\right)\]
%\[\implies  T_c \geq \frac{1}{\epsilon^2_1 E[A_{I_t}(t)]}\ln \left(\frac{12K}{\delta}\right) \]
%\[\implies  T_c \geq \frac{1}{\epsilon^2_1 \theta}\ln \left(\frac{12K}{\delta}\right) \]
%
%and 
%
%\[ \sum\limits_{t=1}^{T_c} A_{I_t}(t) \geq \frac{1}{2}\cdot T_c\cdot E[A_{I_t}(t)] \geq C_3\]
%\[\implies \frac{1}{2}\cdot T_c\cdot E[A_{I_t}(t)] \geq \frac{1}{2\epsilon^2_2}\ln \left(\frac{24K}{\delta}\right)  \]
%\[\implies  T_c \geq \frac{1}{\epsilon^2_2 E[A_{I_t}(t)]}\ln \left(\frac{24K}{\delta}\right) \]
%\[\implies  T_c \geq \frac{1}{\epsilon^2_2 \theta}\ln \left(\frac{24K}{\delta}\right) \]
%
%\[T_{NE} = max\left(\frac{8}{\theta} \cdot \ln \left(\frac{18K}{\delta}\right),\frac{1}{\epsilon^2_1 \theta}\ln \left(\frac{12K}{\delta}\right),\frac{1}{\epsilon^2_2 \theta}\ln \left(\frac{24K}{\delta}\right)\right)\]
%\\
%$E$ - event that all SUs have observed atleast $C_2$ times the selected channel was free \\ 
%$F$ - event that all SUs have correct estimate of $J$.\\
%$D$ - event that all SUs have correct estimate of $N$.  \\
%
%
%\begin{align*}
%Pr(DF) &= 1 - Pr(\overline{DF})  \\
%	&= 1 - Pr(\overline{D})-Pr(\overline{F})   \\
%     &= 1 - Pr(\overline{D}/EF)Pr(EF) - Pr(\overline{D}/\overline{EF})Pr(\overline{EF})-\\&Pr(\overline{F}) \\ 
%     &\geq 1-Pr(\overline{D}/EF)-Pr(\overline{EF})-Pr(\overline{F}) \\
%     &\geq 1-Pr(\overline{D}/EF)-Pr(\overline{E})-2Pr(\overline{F})\\
%     &\geq 1-Pr(\overline{D}/EF)-Pr(\overline{E})-2Pr(\overline{F}/E)Pr(E)-\\&2Pr(\overline{F}/\overline{E})Pr(\overline{E})\\
%     &\geq 1-Pr(\overline{D}/EF)-Pr(\overline{E})-2Pr(\overline{F}/E)-2Pr(\overline{E})\\
%     &\geq 1-Pr(\overline{D}/EF)-2Pr(\overline{F}/E)-3Pr(\overline{E})\\
%     &\geq 1 - \frac{\delta}{6}-\frac{2\delta}{12}-\frac{3\delta}{18}\geq 1 - \frac{\delta}{2} \\
%\end{align*}
%Finally, if $T_{NE} = max\left(\frac{8}{\theta} \cdot \ln \left(\frac{18K}{\delta}\right),\frac{1}{\epsilon^2_1 \theta}\ln \left(\frac{12K}
%{\delta}\right),\frac{1}{\epsilon^2_2 \theta}\ln \left(\frac{24K}{\delta}\right)\right)$ then for $T_c \geq T_{NE}$, all SUs would have 
%correct estimate of $N$ and $J$ with probability atleast $1-\frac{\delta}{2}$. 
%\newline
%For $A$,$D$ and $F$ be as defined previously,
%\begin{align*}
%Pr(ADF)&= 1-Pr(\overline{ADF}) \\
%      &\geq 1 - Pr(\overline{A}) - Pr(\overline{DF})\\
%      &\geq 1 -  \frac{\delta}{2}-\frac{\delta}{2}\\
%      &\geq 1-\delta 
%\end{align*}
%Hence if $T_c = max (T_{NE},T_{CR})$, then with probability $1-\delta$, all SUs would have $\epsilon$-correct channel ranking as well as correct estimate of $N$ given $J$.
%
%
%%\noindent
%%The lemma is derived using the Hoeffding's inequality and Chernoff bound. Hoeffding's inequality is used to derive the number of channel observations (busy or idle) and collisions required to get the correct channel raking as well as estimates of $N$ and $J$. Chernoff bound is used to get the number of slots needed to get those many collisions and channel observations. Note that our proof differs from the regret proof of MC algorithms. In the setting of MC algorithm, channels are always idle, whereas in our case they are not always idle due to the presence of PUs. For more details see \cite{TechReport}.
%
%
%
%
%
%The following theorem states a high confidence bound on the expected regret of CDJ.  The expectation is over the algorithm's randomness. 
\begin{thm}\label{thm:t1}
For all $\Delta > \epsilon, \gamma \in (0, 0.5)$ and $\delta \in [0,1]$, with probability at least $1-\delta$, the expected regret of $N$ SUs using CDJ in the 
	presence of $J$ jammers with $T_C$ slots of learning is upper bounded by $NT_C + N^2exp(1)$, where $T_C$ is 
\begin{equation*}
\label{eq:TCLengh}
 \mbox{round} \bigg(max\bigg(\frac{8}{\theta} \cdot \ln \left(\frac{18K}{\delta}\right),\frac{1}{\epsilon^2_1 \theta}\ln \left(\frac{12K}{\delta}\right),
 \frac{1}{\epsilon^2_2 \theta}\ln \left(\frac{24K}{\delta}\right), 
\end{equation*}	
\begin{equation}
\label{eq:TCLengh}
8K \ln \left(\frac{4K^2}{\delta}\right),\frac{4K}{\epsilon^2}\ln \left( \frac{8 K^2}{\delta} \right) \bigg)\bigg)
\end{equation}	
with $\epsilon_1=\gamma/2K\exp(1)$ and $\epsilon_2= \gamma/K$.
\end{thm}
%\noindent
%The first term ($NT_C$) is the total regret incurred by all users in the CR1 phase. This phase runs for $T_C$ number of time slots, required for estimating correct channel ranking, number of the SUs and Jammers. The second part ($N^2exp(1)$) corresponds to regret incurred in the final OR phase. \\
%\noindent \textbf{Proof:} After estimating $N,J$ and channel ranking from lemma \ref{thm:le1}, all SUs run the OR subroutine for the second time. We will compute the maximum slots required such that all SUs get orthogonalized and start sequential hopping. Our approach to bound regret is similar to approach in \cite{MC}. Probability of collision for any SU at any round $t$ is given by: 
%\begin{align*}
%p_{nc} &= \sum\limits_{k=1}^{N} \frac{1-p_k}{N+m} \left(1-\frac{J}{N}\right)\left(1-\frac{1}{N+m}\right)^{N-1}  \\
%	&+ \sum\limits_{k=N+1}^{N+m} \frac{1-p_k}{N+m} \left(1-\frac{1}{N+m}\right)^{N-1}+ \sum\limits_{k=1}^{N+m} \frac{p_k}{N+m}\\		
%p_{nc} &\geq \sum\limits_{k=1}^{N+m} \frac{1-p_k}{N+m} \left(1-\frac{J}{N}\right)\left(1-\frac{1}{N+m}\right)^{N-1}\\								
%p_{nc} &\geq \left(1-\frac{J}{N}\right)\left(1-\frac{1}{N+m}\right)^{N-1} \sum\limits_{k=1}^{N+m} \frac{1-p_k}{N+m}\\	
%p_{nc} &\geq \left(\frac{N-J}{N}\right)\left(1-\frac{1}{N+m}\right)^{N-1} \theta \\
%p_{nc} &\geq \left(\frac{1}{N}\right)\left(1-\frac{1}{N+m}\right)^{N+m-1} \theta \\
%p_{nc} &\geq \frac{\theta}{Nexp(1)}\\
%%&\sum\limits_{k=1}^{N+m} \frac{1-p_k}{N+m} 
%%\geq \sum\limits_{k=1}^{N+m} \frac{1-p_k}{K} \\
%\end{align*}
%
%Therefore probability of no collision $p_{nc} > \frac{\theta}{Nexp(1)}$. Let $X$ be a geometric random variable with success probability $p_{nc}$. Therefore, expected number of slots $T_f$ for first success is given by :
%\[T_f = \frac{1}{p_{nc}}\] 
%\[\implies T_f < \frac{Nexp(1)}{\theta} \]  
%
%Let $r_{i,t}$ be an indicator variable which equals 1 if player i incurred regret at round t and 0
%otherwise. 
%We will now bound the expected regret due to players when running the OR subroutine for second time.
%\begin{small}
%   \[Regret \leq E\left[\sum\limits_{t=T_L+1}^{T} \sum\limits_{i=1}^{N}r_{i,t} \right]\]
%   \[Regret \leq E\left[\sum\limits_{t=T_L+1}^{T} \sum\limits_{i=1}^{N}\mathbbm{1}\{SU \ i \ not \ orthogonalized \ at \ round \ t\} \right]\]
%  \[Regret \leq E\left[\sum\limits_{t=T_L+1}^{T} N.\mathbbm{1}\{SU \ i \ not \ orthogonalized \ at \ round \ t\} \right]\]
%  \[Regret \leq N.T_f\]
%  \begin{equation} \label{eq:r} Regret \leq \frac{N^2exp(1)}{\theta}\end{equation} 
%\end{small}
%Using lemma \ref{thm:le1} and Eq. (\ref{eq:r}) we prove that channel ranking, number of SUs and jammers can be estimated with probability $1-\delta$
%and total regret is bounded by $NT_L + \frac{N^2exp(1)}{\theta}$.
%Hence proving theorem \ref{thm:t1}.

%The proof of the theorem is based on the following lemma.








